Updated model-independent measurement of the strong-phase differences between $D^0$ and $\bar{D}^0 \to K^{0}_{S/L}\pi^+\pi^-$ decays

The strong-phase differences between $D^0\to K_{S/L}^0\pi^+\pi^-$ and $\bar{D}^0\to K_{S/L}^0\pi^+\pi^-$ decays are one of the most important inputs in measuring the $C\!P$ violating angle $\gamma$ via $B^- \to D K^-$ decays. They also play a key role in studies of charm mixing and indirect $C\!P$ violation. In this paper, the strong-phase differences are determined in a model-independent way with quantum-correlated $D^0$-$\bar{D}^0$ decays from 7.93 fb$^{-1}$ of $e^+e^-$ annihilation data at $\sqrt{s}$=3.773 GeV by the BESIII experiment. These results are the most precise to date and are expected to significantly reduce associated uncertainties in determining the $C\!P$ violating angle $\gamma$ and related charm mixing parameters.

==> body/acknowledgement_2025-02-06.tex <==
%% Saved at => 2025-02-06
\section{Acknowledgement}

The BESIII Collaboration thanks the staff of BEPCII (https://cstr.cn/31109.02.BEPC) and the IHEP computing center for their strong support. This work is supported in part by National Key R\&D Program of China under Contracts Nos.2023YFA1606000, 2023YFA1606704; National Natural Science Foundation of China (NSFC) under Contracts Nos. 11635010, 11935015, 11935016, 11935018, 12025502, 12035009, 12035013, 12061131003, 12192260, 12192261, 12192262, 12192263, 12192264, 12192265, 12221005, 12225509, 12235017, 12361141819, 12405112; the Chinese Academy of Sciences (CAS) Large-Scale Scientific Facility Program; CAS under Contract No. YSBR-101; 100 Talents Program of CAS; The Institute of Nuclear and Particle Physics (INPAC) and Shanghai Key Laboratory for Particle Physics and Cosmology; Agencia Nacional de Investigación y Desarrollo de Chile (ANID), Chile under Contract No. ANID PIA/APOYO AFB230003; German Research Foundation DFG under Contract No. FOR5327; Istituto Nazionale di Fisica Nucleare, Italy; Knut and Alice Wallenberg Foundation under Contracts Nos. 2021.0174, 2021.0299; Ministry of Development of Turkey under Contract No. DPT2006K-120470; National Research Foundation of Korea under Contract No. NRF-2022R1A2C1092335; National Science and Technology fund of Mongolia; National Science Research and Innovation Fund (NSRF) via the Program Management Unit for Human Resources \& Institutional Development, Research and Innovation of Thailand under Contract No. B50G670107; Polish National Science Centre under Contract No. 2024/53/B/ST2/00975; Swedish Research Council under Contract No. 2019.04595; U. S. Department of Energy under Contract No. DE-FG02-05ER41374



